Unsupervised Novelty Detection Methods Benchmarking with Wavelet Decomposition

Novelty detection is a critical task in various engineering fields. Numerous approaches to novelty detection rely on supervised or semi-supervised learning, which requires labelled datasets for training. However, acquiring labelled data, when feasible, can be expensive and time-consuming. For these reasons, unsupervised learning is a powerful alternative that allows performing novelty detection without needing labelled samples. In this study, numerous unsupervised machine learning algorithms for novelty detection are compared, highlighting their strengths and weaknesses in the context of vibration sensing. The proposed framework uses a continuous metric, unlike most traditional methods that merely flag anomalous samples without quantifying the degree of anomaly. Moreover, a new dataset is gathered from an actuator vibrating at specific frequencies to benchmark the algorithms and evaluate the framework. Novel conditions are introduced by altering the input wave signal. Our findings offer valuable insights into the adaptability and robustness of unsupervised learning techniques for real-world novelty detection applications.

==> Sections/abbr.tex <==
\begin{supertabular}{ll}
ACO & Ant Colony Optimization \\
AI & Artificial Intelligence \\
CBLOF & Cluster-Based Local Outlier Factor\\
CNN & Convolutional Neural Network \\
CWRU & Case Western Reserve University\\
FP & Feature Percentage \\
GMM & Gaussian Mixture Model \\
IF & Isolation Forest \\
IMS & Intelligent Maintenance Systems\\
LOF & Local Outlier Factor\\
MFCC & Mel-frequency Cepstral Coeﬃcients\\
ML & Machine Learning \\
MSE & Mean Squared Error \\
NM & Novelty Metric\\
nuSVM & one-class Support Vector Machine \\
PCA & Principal Component Analysis \\
P2P & Peak-to-Peak \\
RMS & Root-Mean-Square \\
RSGWPT & Redundant Second Generation\\
&Wavelet Packet Transform\\
SOM & Self-Organizing Maps\\
SPCP & Self-Priming Centrifugal Pump\\
STD & Standard Deviation \\
SVM & Support Vector Machine\\
TSF & Traditional Statistical Features\\
UML & Unsupervised Machine Learning \\
WPD & Wavelet Packet Decomposition\\
\end{supertabular}

==> Sections/bibitems.tex <==
\bibitem{Chalouli2017}Chalouli, M., Berrached, N. \& Denai, M. Intelligent Health Monitoring of Machine Bearings Based on Feature Extraction. {\em Journal Of Failure Analysis And Prevention}. \textbf{17}, 1053-1066 (2017,10), https://doi.org/10.1007/s11668-017-0343-y
\bibitem{Mansour2023}Mansour, R., Abdel-Khalek, S., Hilali-Jaghdam, I., Nebhen, J., Cho, W. \& Joshi, G. An intelligent outlier detection with machine learning empowered big data analytics for mobile edge computing. {\em Cluster Computing}. \textbf{26}, 71-83 (2023,2), https://doi.org/10.1007/s10586-021-03472-4
\bibitem{SPYTEK2023109823}Spytek, J., Machynia, A., Dziedziech, K., Dworakowski, Z. \& Holak, K. Novelty detection approach for the monitoring of structural vibrations using vision-based mean frequency maps. {\em Mechanical Systems And Signal Processing}. \textbf{185} pp. 109823 (2023), https://www.sciencedirect.com/science/article/pii/S0888327022008913
\bibitem{Zhou2019}Zhou, Q., Shen, H., Zhao, J., Liu, X. \& Xiong, X. Degradation State Recognition of Rolling Bearing Based on K-Means and CNN Algorithm. {\em Shock And Vibration}. \textbf{2019}, 8471732 (2019), https://onlinelibrary.wiley.com/doi/abs/10.1155/2019/8471732
\bibitem{IMS_data}Lee, J., Qiu, H., Yu, G., Lin, J. \& Services, R. Bearing Data Set. (IMS, University of Cincinnati, NASA Prognostics Data Repository, NASA Ames Research Center, Moffett Field, CA,2007)
\bibitem{Pinedo2020}Pinedo-Sánchez, L., Mercado-Ravell, D. \& Carballo-Monsivais, C. Vibration analysis in bearings for failure prevention using CNN. {\em Journal Of The Brazilian Society Of Mechanical Sciences And Engineering}. \textbf{42}, 628 (2020,11), https://doi.org/10.1007/s40430-020-02711-w
\bibitem{ZHANG2018}Zhang, Y., Li, X., Gao, L. \& Li, P. A new subset based deep feature learning method for intelligent fault diagnosis of bearing. {\em Expert Systems With Applications}. \textbf{110} pp. 125-142 (2018), https://www.sciencedirect.com/science/article/pii/S0957417418303324
\bibitem{Gattino2023}Gattino, C., Ottonello, E., Baggetta, M., Razzoli, R., Stecki, J. \& Berselli, G. Application of AI failure identification techniques in condition monitoring using wavelet analysis. {\em The International Journal Of Advanced Manufacturing Technology}. \textbf{125}, 4013-4026 (2023,4), https://doi.org/10.1007/s00170-022-10549-w
\bibitem{Masud2011}Masud, M., Gao, J., Khan, L., Han, J. \& Thuraisingham, B. Classification and Novel Class Detection in Concept-Drifting Data Streams under Time Constraints. {\em IEEE Transactions On Knowledge And Data Engineering}. \textbf{23}, 859-874 (2011)
\bibitem{Breunig00}Breunig, M., Kröger, P., Ng, R. \& Sander, J. LOF: Identifying Density-Based Local Outliers.. {\em ACM Sigmod Record}. \textbf{29} pp. 93-104 (2000,6)
\bibitem{HE2003}He, Z., Xu, X. \& Deng, S. Discovering cluster-based local outliers. {\em Pattern Recognition Letters}. \textbf{24}, 1641-1650 (2003), https://www.sciencedirect.com/science/article/pii/S0167865503000035
\bibitem{Clifton06}Clifton, D., Bannister, P. \& Tarassenko, L. Learning Shape for Jet Engine Novelty Detection. {\em Advances In Neural Networks - ISNN 2006}. pp. 828-835 (2006)
\bibitem{Garcia19}Garcia, K., Poel, M., Kok, J. \& Carvalho, A. Online Clustering for Novelty Detection and Concept Drift in Data Streams. {\em Progress In Artificial Intelligence}. pp. 448-459 (2019)
\bibitem{Wan21}Wan, L., Zhang, G., Li, H. \& Li, C. A Novel Bearing Fault Diagnosis Method Using Spark-Based Parallel ACO-K-Means Clustering Algorithm. {\em IEEE Access}. \textbf{9} pp. 28753-28768 (2021)
\bibitem{CWRU_data}University, C. Bearing Data Center: Seeded Fault Test Data. (Case School of Engineering, Case Western Reserve University), http://data-acquisition.case.edu/, Accessed: 2024-06-05


==> Tabs/aeaugparam.tex <==
% \usepackage{color}
% \usepackage[normalem]{ulem}
% \usepackage{tabularray}
\definecolor{Shark}{rgb}{0.129,0.145,0.16}
\begin{table}
\label{tab:aeaugparam}
\centering
\begin{tblr}{
  row{even} = {c},
  row{1} = {c},
  row{5} = {c},
  row{7} = {c},
  cell{2}{2} = {fg=Shark},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  hlines,
  hline{1,8} = {-}{0.08em},
}
\textbf{Model} & $\mathbf{N_{E1},N_{D1}}$ & $\mathbf{N_{E2}}$ & $\mathbf{lr}$ & $\mathbf{bs}$ \\
KMeans       & $80$                         & $85$\textcolor[rgb]{0.129,0.145,0.161}{} & $0.08$\textcolor[rgb]{0.129,0.145,0.161}{} & $64$        \\
DBSCAN       & $75$                         & $85$                                     & $0.2$                                      & $32$        \\
GMM          & $79$                         & $85$                                     & $0.08$                                     & $32$        \\
nuSVM        & $80$                         & $93$                                     & $0.09$                                     & $32$        \\
IForest      & $79$                         & $85$                                     & $0.02$                                     & $64$        \\
LOF          & $79$                         & $88$                                     & $0.03$                                     & $32$        
\end{tblr}
\end{table}

==> Tabs/aeredparam.tex <==
% \usepackage{color}
% \usepackage[normalem]{ulem}
% \usepackage{tabularray}
\definecolor{Shark}{rgb}{0.129,0.145,0.16}
\begin{table}
\label{tab:aeredparam}
\centering
\begin{tblr}{
  row{even} = {c},
  row{1} = {c},
  row{5} = {c},
  row{7} = {c},
  cell{2}{2} = {fg=Shark},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  hlines,
  hline{1,8} = {-}{0.08em},
}
\textbf{Model} & $\mathbf{N_{E1},N_{D1}}$ & $\mathbf{N_{E2}}$ & $\mathbf{lr}$ & $\mathbf{bs}$ \\
$KMeans$& $61$& $32$& $0.03$& $64$\\
$DBSCAN$& $56$& $10$& $0.08$& $64$\\
$GMM$& $61$& $10$& $0.01$& $64$\\
$nuSVM$& $65$& $10$& $0.1$& $64$\\
$IForest$& $50$& $45$& $0.03$& $64$\\
$LOF$& $50$& $10$& $0.01$& $32$        
\end{tblr}
\end{table}



==> Tabs/pcaparam.tex <==
% \usepackage{color}
% \usepackage[normalem]{ulem}
% \usepackage{tabularray}
\definecolor{Shark}{rgb}{0.129,0.145,0.16}
\begin{table}
\label{tab:pcaparam}
\centering
\begin{tblr}{
  cells = {c},
  cell{2}{2} = {fg=Shark},
  hlines,
  hline{1,3} = {-}{0.08em},
}
\textbf{Model} & \textbf{N\_\{E1\},N\_\{D1\}} & \textbf{N\_\{E2\}}                       & \textbf{lr}                                & \textbf{bs} \\
$PCA$          & $80$                         & $85$\textcolor[rgb]{0.129,0.145,0.161}{} & $0.08$\textcolor[rgb]{0.129,0.145,0.161}{} & $64$        
\end{tblr}
\end{table}
